Adaptive Application Behaviour for Robot Swarms using Mixed-Criticality

Communication is a vital component for all swarm robotics applications, and even simple swarm robotics behaviours often break down when this communication is unreliable. Since wireless communications are inherently subject to interference and signal degradation, real-world swarm robotics applications will need to be able handle such scenarios. This paper argues for tighter integration of application level and network layer behaviour, so that the application can alter its behaviour in response to a degraded network. This is systematised through the implementation of a mixed-criticality system model. We compare a static application behaviour with that of an application that is able to alter its behaviour in response to the current criticality level of a mixed-criticality wireless protocol. Using simulation results we show that while a static approach is sufficient if the network conditions are known a priori, a mixed-criticality system model is able to adapt application behaviour to better support unseen or unpredictable conditions.

==> eptcsdata.tex <==
\providecommand{\firstpage}{71}
\providecommand{\publicationstatus}{A. Ferrando, R.C. Cardoso (Eds.): Third Workshop on\\ Agents and Robots for reliable Engineered Autonomy 2023 (AREA'23)\\
EPTCS 391, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.391.9}{10.4204/EPTCS.391.9}}
\pdfoutput=1

